Statistical Study of Emerging Flux Regions and the Upper Atmosphere Response

We statistically study the property of emerging flux regions (EFRs) and the upper solar atmosphere response to the flux emergence by using data from the Helioseismic and Magnetic Imager (HMI) and the Atmospheric Imaging Assembly (AIA) on board the Solar Dynamics Observatory (SDO). Parameters including the total emerged flux, the flux growth rate, the maximum area, the duration of the emergence and the separation speed of the opposite polarities are adopted to delineate the property of the EFRs. The response of the upper atmosphere is addressed by the response of the atmosphere at different wavelengths (and thus at different temperatures). According to our results, the total emerged fluxes are in the range of (0.44 -- 11.2)$\times10^{19}$ Mx while the maximum area ranges from 17 to 182 arcsec$^2$. The durations of the emergence are between 1 and 12 hours, which are positively correlated to both the total emerged flux and the maximum area. The maximum distances between the opposite polarities are 7 -- 25 arcsec and are also correlated to the duration positively. The separation speeds are from 0.05 to 1.08 km s$^{-1}$, negatively correlated to the duration. The derived flux growth rates are (0.1 -- 1.3)$\times10^{19}$ Mx hr$^{-1}$, which are positively correlated to the total emerging flux. The upper atmosphere responds to the flux emergence in the 1600\AA\ chromospheric line first, and then tens and hundreds of seconds later, in coronal lines, such as the 171\AA\ (T=10$^{5.8}$ K) and 211\AA\ (T=10$^{6.3}$ K) lines almost simultaneously, suggesting the successively heating of atmosphere from the chromosphere to the corona.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

